Modeling Information Cascades with Self-exciting Processes via Generalized Epidemic Models

Epidemic models and self-exciting processes are two types of models used to describe diffusion phenomena online and offline. These models were originally developed in different scientific communities, and their commonalities are under-explored. This work establishes, for the first time, a general connection between the two model classes via three new mathematical components. The first is a generalized version of stochastic Susceptible-Infected-Recovered (SIR) model with arbitrary recovery time distributions; the second is the relationship between the (latent and arbitrary) recovery time distribution, recovery hazard function, and the infection kernel of self-exciting processes; the third includes methods for simulating, fitting, evaluating and predicting the generalized process. On three large Twitter diffusion datasets, we conduct goodness-of-fit tests and holdout log-likelihood evaluation of self-exciting processes with three infection kernels --- exponential, power-law and Tsallis Q-exponential. We show that the modeling performance of the infection kernels varies with respect to the temporal structures of diffusions, and also with respect to user behavior, such as the likelihood of being bots. We further improve the prediction of popularity by combining two models that are identified as complementary by the goodness-of-fit tests.

==> sections/related_work.tex <==
\section{Related Work}
In this section, we summarize some relevant work from literature about stochastic SIR and information diffusion modeling.

A notable amount of effort has been put into generalizing epidemic models in terms of both the infection time interval distribution and the recovery time interval distribution in epidemiological study. 
\citet{keeling1997disease} reformulate the deterministic epidemic models as integro-differential equations to impose a normal distribution for infectious periods, while a Weibull distributed infection time intervals is introduced to the stochastic SIR model in \citep{streftaris2012non}. 
Another formulation of the SIR model captures arbitrary infection and recovery time interval distributions within a network by incorporating the idea of message passing algorithms \citep{karrer2010message}. 
Besides studies from epidemiology, epidemic models have also been applied to model event data from online social media platforms such as Twitter in a range of studies \citep{martin2016exploring,goel2015note}. 
\citet{kimura2009efficient} first apply the simplest SIS model, which allows notes to be activated multiple times, to study information diffusion in a network. \citet{jin2013epidemiological} use an enhanced SEIZ (susceptible, exposed, infected, skeptic) model, which introduces an extra exposed state (E) to the SIR model for capturing a incubation period, to detect rumors from Twitter cascades. 

Hawkes processes model have attracted a great research attention with regard to social media analysis because of its explainability and modeling capability as a generative model. \citet{Mishra2016FeaturePrediction} model temporal diffusion data with some fine-grained features and stack another prediction layer for popularity prediction. \citet{luo2015multi} employ a multi-variate Hawkes processes model with an imposed structural constraints for modeling multiple event sequences. \citet{Rizoiu2017c} propose a finite population restricted Hawkes processes model which is then linked to the stochastic SIR model.

However, these work do not link the generalized epidemic models to point process models for information diffusion modeling.
